Well-balanced convex limiting for finite element discretizations of steady convection-diffusion-reaction equations

We address the numerical treatment of source terms in algebraic flux correction schemes for steady convection-diffusion-reaction (CDR) equations. The proposed algorithm constrains a continuous piecewise-linear finite element approximation using a monolithic convex limiting (MCL) strategy. Failure to discretize the convective derivatives and source terms in a compatible manner produces spurious ripples, e.g., in regions where the coefficients of the continuous problem are constant and the exact solution is linear. We cure this deficiency by incorporating source term components into the fluxes and intermediate states of the MCL procedure. The design of our new limiter is motivated by the desire to preserve simple steady-state equilibria exactly, as in well-balanced schemes for the shallow water equations. The results of our numerical experiments for two-dimensional CDR problems illustrate potential benefits of well-balanced flux limiting in the scalar case.

==> images/balanced_reaction_tv.tex <==
\begin{tikzpicture}[scale=0.7]
\begin{semilogxaxis}[ legend pos=north west, ylabel = \Large{TV($u_h$)}, xlabel = \Large{$\#$dofs},
    legend cell align ={left}, 
     legend style={nodes={scale=0.75, transform shape}}]
\addplot[color=crimson,  mark=square*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 25.0 , 100.277 )( 81.0 , 271.547 )( 289.0 , 565.148 )( 1089.0 , 1155.04 )( 4225.0 , 2334.48 )( 16641.0 , 4709.61 )( 66049.0 , 9483.67 )};
\addlegendentry{WMC+Grid~1} 
\addplot[color=crimson,  mark=oplus*, line width = 0.5mm, dotted,,mark options = {scale= 1.5, solid}]
coordinates{( 41.0 , 150.348 )( 145.0 , 320.562 )( 545.0 , 665.724 )( 2113.0 , 1347.42 )( 8321.0 , 2734.51 )( 33025.0 , 5527.01 )( 131585.0 , 11250 )};
\addlegendentry{WMC+Grid~2} 
\addplot[color=navy_blue,  mark=square*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 25.0 , 105.741 )( 81.0 , 279.269 )( 289.0 , 580.296 )( 1089.0 , 1187.32 )( 4225.0 , 2384.26 )( 16641.0 , 4789.5 )( 66049.0 , 9567.75 )};
\addlegendentry{MC+Grid~1} 
\addplot[color=navy_blue,  mark=oplus*, line width = 0.5mm, dotted,,mark options = {scale= 1.5, solid}]
coordinates{( 41.0 , 152.14 )( 145.0 , 329.732 )( 545.0 , 690.166 )( 2113.0 , 1400.63 )( 8321.0 , 2840.76 )( 33025.0 , 5685.87 )( 131585.0 , 11371.2 )};
\addlegendentry{MC+Grid~2} 
\end{semilogxaxis}
\end{tikzpicture}


==> images/boundary_layer_tv_var_eps.tex <==
\begin{tikzpicture}[scale=0.7]
\begin{semilogxaxis}[ legend pos=north west, ylabel = \Large{TV($u_h$)}, xlabel = \Large{$\#$dofs},
    legend cell align ={left}, 
     legend style={nodes={scale=0.75, transform shape}}]
\addplot[color=crimson,  mark=diamond*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 25.0 , 13.7386 )( 81.0 , 38.4283 )( 289.0 , 90.231 )( 1089.0 , 194.456 )( 4225.0 , 402.146 )( 16641.0 , 819.507 )( 66049.0 , 1664.61 )};
\addlegendentry{WMC+$\varepsilon=10^{-3}$} 
\addplot[color=crimson,  mark=pentagon*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 25.0 , 13.7774 )( 81.0 , 38.5937 )( 289.0 , 90.8932 )( 1089.0 , 197.098 )( 4225.0 , 410.322 )( 16641.0 , 837.071 )( 66049.0 , 1690.72 )};
\addlegendentry{WMC+$\varepsilon=10^{-6}$} 
\addplot[color=crimson,  mark=triangle*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 25.0 , 13.7775 )( 81.0 , 38.5939 )( 289.0 , 90.8938 )( 1089.0 , 197.101 )( 4225.0 , 410.333 )( 16641.0 , 837.112 )( 66049.0 , 1690.9 )};
\addlegendentry{WMC+$\varepsilon=10^{-9}$} 
\addplot[color=navy_blue,  mark=diamond*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 25.0 , 20.4659 )( 81.0 , 51.971 )( 289.0 , 108.686 )( 1089.0 , 218.625 )( 4225.0 , 432.8 )( 16641.0 , 856.791 )( 66049.0 , 1697.01 )};
\addlegendentry{MC+$\varepsilon=10^{-3}$} 
\addplot[color=navy_blue,  mark=pentagon*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 25.0 , 20.4965 )( 81.0 , 52.0768 )( 289.0 , 109.043 )( 1089.0 , 219.833 )( 4225.0 , 440.722 )( 16641.0 , 882.195 )( 66049.0 , 1764.74 )};
\addlegendentry{MC+$\varepsilon=10^{-6}$} 
\addplot[color=navy_blue,  mark=triangle*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 25.0 , 20.4965 )( 81.0 , 52.0769 )( 289.0 , 109.044 )( 1089.0 , 219.834 )( 4225.0 , 440.727 )( 16641.0 , 882.213 )( 66049.0 , 1764.81 )};
\addlegendentry{MC+$\varepsilon=10^{-9}$} 
\end{semilogxaxis}
\end{tikzpicture}


==> images/circular_convection_max_min.tex <==
\begin{tikzpicture}[scale=0.8]
\begin{semilogxaxis}[
    legend pos=north east, xlabel = \Large{$\#\ \mathrm{dof}$}, ylabel=\Large{$\mathrm{osc}_u\left(u_h\right)$},
    legend cell align ={left},,
    legend style={nodes={scale=0.75, transform shape}}]
\addplot[color=crimson,  mark=square*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 25.0 , 0.0 )( 81.0 , 0.0 )( 289.0 , 0.0 )( 1089.0 , 0.0 )( 4225.0 , 6.227418580806443e-11 )( 16641.0 , 6.1026739217595605e-12 )};
\addlegendentry{MC+Grid~1} 
\addplot[color=crimson,  mark=oplus*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 145.0 , 0.0 )( 545.0 , 1.3670398146814478e-11 )( 2113.0 , 2.220446049250313e-16 )( 8321.0 , 1.2165091156646213e-10 )( 33025.0 , 2.5308456219619302e-08 )( 131585.0 , 4.639361023328625e-05 )};
\addlegendentry{MC+Grid~2} 
\addplot[color=azure,  mark=square*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 25.0 , 0.0 )( 81.0 , 0.0 )( 289.0 , 0.0 )( 1089.0 , 0.0 )( 4225.0 , 0.0 )( 16641.0 , 1.8382240174474873e-09 )};
\addlegendentry{MU+Grid~1} 
\addplot[color=azure,  mark=oplus*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 145.0 , 0.0 )( 545.0 , 0.1444293802179999 )( 2113.0 , 0.0021944939919900097 )( 8321.0 , 0.03736927917199995 )( 33025.0 , 0.006841644508050138 )( 131585.0 , 0.0026159733337673963 )};
\addlegendentry{MU+Grid~2} 
\end{semilogxaxis}
\end{tikzpicture}


==> images/iterations_two_layers.tex <==
\begin{tikzpicture}[scale=0.8]
\begin{semilogxaxis}[scaled y ticks = false, axis y line*=left,xticklabels={,,},
    legend pos=north west, ylabel = \Large{iterations+rejections},
    legend cell align ={left}, 
     legend style={nodes={scale=0.75, transform shape}}]
\addplot[color=crimson,  mark=square*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 289.0 , 90.0 )( 1089.0 , 157.0 )( 4225.0 , 131.0 )( 16641.0 , 118.0 )( 66049.0 , 156.0 )};\label{TL_MCL_1}
\addplot[color=crimson,  mark=oplus*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}] 
coordinates{( 145.0 , 63.0 )( 545.0 , 158.0 )( 2113.0 , 392.0 )( 8321.0 , 569.0 )( 33025.0 , 1613.0 )};\label{TL_MCL_2}
\end{semilogxaxis}
\begin{semilogxaxis}[scaled y ticks = false, axis y line*=right,
    legend pos=north west, xlabel =  \Large{$\#\ \mathrm{dof}$}, 
    legend cell align ={left},
     legend style={nodes={scale=0.75, transform shape}}]
\addlegendimage{/pgfplots/refstyle=TL_MCL_1}\addlegendentry{MC+Grid~1}
\addlegendimage{/pgfplots/refstyle=TL_MCL_2}\addlegendentry{MC+Grid~2}
\addplot[color=azure,  mark=square*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}]
coordinates{( 289.0 , 59.0 )( 1089.0 , 102.0 )( 4225.0 , 132.0 )( 16641.0 , 115.0 )( 66049.0 , 120.0 )};
\addlegendentry{MU+Grid~1} 
\addplot[color=azure,  mark=oplus*, line width = 0.5mm, dashdotted,,mark options = {scale= 1.5, solid}] 
coordinates{( 145.0 , 34.0 )( 545.0 , 63.0 )( 2113.0 , 99.0 )( 8321.0 , 109.0 )( 33025.0 , 94.0 )};
\addlegendentry{MU+Grid~2} 
\end{semilogxaxis}
\end{tikzpicture}


==> images/smear_two_layers.tex <==
\begin{tikzpicture}[scale=0.8]
\begin{semilogxaxis}[
    legend pos=north east, xlabel = \Large{$\#\ \mathrm{dof}$}, ylabel=\Large{$\mathrm{smear}_{\mathrm{int}}$},
    legend cell align ={left},,
    legend style={nodes={scale=0.75, transform shape}}]
\addplot[color=crimson,  mark=square*, line width = 0.5mm,dashdotted,, mark options = {scale= 1.5, solid}] 
coordinates{( 289.0 , 0.143475 )( 1089.0 , 0.0869041 )( 4225.0 , 0.0517937 )( 16641.0 , 0.028997 )( 66049.0 , 0.015762 )};
\addlegendentry{MC+Grid~1} 
\addplot[color=crimson,  mark=oplus*, line width = 0.5mm,dashdotted,, mark options = {scale= 1.5, solid}] 
coordinates{( 145.0 , 0.135583 )( 545.0 , 0.0686695 )( 2113.0 , 0.0440025 )( 8321.0 , 0.0260989 )( 33025.0 , 0.0146098 )};
\addlegendentry{MC+Grid~2} 
\addplot[color=azure,  mark=square*, line width = 0.5mm,dashdotted,, mark options = {scale= 1.5, solid}] 
coordinates{( 289.0 , 0.135798 )( 1089.0 , 0.0813702 )( 4225.0 , 0.0482704 )( 16641.0 , 0.0273206 )( 66049.0 , 0.0149734 )};
\addlegendentry{MU+Grid~1} 
\addplot[color=azure,  mark=oplus*, line width = 0.5mm,dashdotted,, mark options = {scale= 1.5, solid}] 
coordinates{( 145.0 , 0.149428 )( 545.0 , 0.064505 )( 2113.0 , 0.039859 )( 8321.0 , 0.0239594 )( 33025.0 , 0.013668 )};
\addlegendentry{MU+Grid~2} 
\end{semilogxaxis}
\end{tikzpicture}


==> new_command.tex <==
\newcommand{\leb}{\mathrm{leb}}
\newcommand{\lgl}{\mathrm{lgl}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bo}{\boldsymbol{0}}
\newcommand{\mk}{\mathtt{k}}
\newcommand{\bA}{\mathrm{\textbf{A}}}
\newcommand{\bB}{\mathrm{\textbf{B}}}
\newcommand{\bC}{\mathrm{\textbf{C}}}
\newcommand{\bL}{\mathrm{\textbf{L}}}
\newcommand{\bG}{\mathrm{\textbf{G}}}
\newcommand{\bF}{\mathrm{\textbf{F}}}
\newcommand{\bQ}{\mathrm{\textbf{Q}}}
\newcommand{\bP}{\mathrm{\textbf{P}}}
\newcommand{\bS}{\mathrm{\textbf{S}}}
\newcommand{\mr}{\mathrm{r}}
\newcommand{\me}{\mathrm{e}}
\newcommand{\mB}{\mathrm{B}}
\newcommand{\sas}{\mathrm{SAS}}
\newcommand{\abso}{\mathrm{abs}}
\newcommand{\sol}{\mathrm{sol}}
\newcommand{\ions}{\mathrm{ions}}
\newcommand{\ses}{\mathrm{SES}}
\newcommand{\sass}{\mathrm{SAS-S}}
\newcommand{\sess}{\mathrm{SES-S}}
\newcommand{\ith}{\mathrm{th}}
\newcommand{\omegaij}{\omega_{ij}^{\eta}}
\newcommand{\ylm}{Y_{\ell m}}
\newcommand{\ylmdash}{Y_{\ell ' m'}}
\newcommand{\clomo}{C_{0\ell_0m_0}^j}
\newcommand{\cik}{C_{\ti\tk}^j}
\newcommand{\fni}{f_n^i}
\newcommand{\ti}{\mathtt{i}}
\newcommand{\tk}{\mathtt{k}}
\newcommand{\te}{\mathtt{e}}
\newcommand{\xni}{\boldsymbol{x}_i^n}
\newcommand{\xnj}{\boldsymbol{x}_j^n}
\newcommand{\vry}{\varrho_{\scriptscriptstyle{Y}}}
%theorem styles
\newsiamremark{remark}{Remark}
\newsiamremark{example}{Example}
